Precise Length Control in Large Language Models

Large Language Models (LLMs) are increasingly used in production systems, powering applications such as chatbots, summarization, and question answering. Despite their success, controlling the length of their response remains a significant challenge, particularly for tasks requiring structured outputs or specific levels of detail. In this work, we propose a method to adapt pre-trained decoder-only LLMs for precise control of response length. Our approach incorporates a secondary length-difference positional encoding (LDPE) into the input embeddings, which counts down to a user-set response termination length. Fine-tuning with LDPE allows the model to learn to terminate responses coherently at the desired length, achieving mean token errors of less than 3 tokens. We also introduce Max New Tokens++, an extension that enables flexible upper-bound length control, rather than an exact target. Experimental results on tasks such as question answering and document summarization demonstrate that our method enables precise length control without compromising response quality.

==> further_work.tex <==
\section{Further Work}
\label{sec:further}
The efficacy of this method lends itself nicely to other tasks beyond simply controlling output length.
The following sections will discuss some ideas for future work that could be studied using the methods discussed so far,
as well as some refinements which could be made to the method itself.


\paragraph{Relative Positional Encoding}
This paper uses an absolute countdown from a predetermined response length to calculate the positional encoding.
Another option would be to use the relative position of each token to the start of the sequence,
as doing so could help the model to better learn the concept of remaining token budget.
Since the positional encoding would always be relative,
the model may be better able to generalise to various response lengths rather than those which it has most seen during training~\cite{kazemnejad2023impact}.


\paragraph{Improving Sample Efficiency}
Using a summarisation dataset consisting of multiple summaries of the same article with different lengths,
for example like the synthetic CNN/DailyMail dataset discussed in Section~\ref{sec:summarisation},
could enable the model to learn the concept of a \enquote{token budget} more efficiently.
This could help minimise any loss of general reasoning ability as a result of the fine-tuning process.
